MIMHD: Accurate and Efficient Hyperdimensional Inference Using Multi-Bit In-Memory Computing

Hyperdimensional Computing (HDC) is an emerging computational framework that mimics important brain functions by operating over high-dimensional vectors, called hypervectors (HVs). In-memory computing implementations of HDC are desirable since they can significantly reduce data transfer overheads. All existing in-memory HDC platforms consider binary HVs where each dimension is represented with a single bit. However, utilizing multi-bit HVs allows HDC to achieve acceptable accuracies in lower dimensions which in turn leads to higher energy efficiencies. Thus, we propose a highly accurate and efficient multi-bit in-memory HDC inference platform called MIMHD. MIMHD supports multi-bit operations using ferroelectric field-effect transistor (FeFET) crossbar arrays for multiply-and-add and FeFET multi-bit content-addressable memories for associative search. We also introduce a novel hardware-aware retraining framework (HWART) that trains the HDC model to learn to work with MIMHD. For six popular datasets and 4000 dimension HVs, MIMHD using 3-bit (2-bit) precision HVs achieves (i) average accuracies of 92.6% (88.9%) which is 8.5% (4.8%) higher than binary implementations; (ii) 84.1x (78.6x) energy improvement over a GPU, and (iii) 38.4x (34.3x) speedup over a GPU, respectively. The 3-bit $\times$ is 4.3x and 13x faster and more energy-efficient than binary HDC accelerators while achieving similar accuracies.

==> preamble.tex <==
\usepackage{times}
\usepackage{tikz}
\usetikzlibrary{positioning}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.3}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{patterns}
% \usepackage{subcaption}
\usepackage{subfiles}
\usepackage{xcolor}
%\usepackage{caption}
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{multirow}
\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))*0.7}%
}

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\pgfplotsset{compat=1.15}

% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}

\usepackage{subfigure}
\usepackage{epstopdf}
\usepackage{epsfig}
% \usepackage{cite}
\usepackage{array}
%\usepackage{fancyhdr}
\usepackage{lipsum}
\usepackage[]{algorithm2e}
\usepackage{tabularx}
%\usepackage{color,soul}
\usepackage{hyperref}
\newcommand{\footremember}[2]{%
    \footnote{#2}
    \newcounter{#1}
    \setcounter{#1}{\value{footnote}}%
}
\newcommand{\footrecall}[1]{%
    \footnotemark[\value{#1}]%
} 

\def\sharedaffiliation{%
\end{tabular}
\begin{tabular}{c}}
%
% \usepackage[margin=0.8in,footskip=0.25in]{geometry}

\usepackage{enumitem}


\usepackage{booktabs} % For formal tables

\usepackage{graphicx}
%\usepackage{subcaption}
\usepackage{booktabs}
%\usepackage{float}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{array}
\usepackage{tabularx}
\usepackage{bm}
\usepackage{soul}
\usepackage{tikz}
\usepackage{amssymb}
\usepackage{amsmath}
% \usepackage{slashbox}
\usepackage{xfrac}
% \usepackage[export]{adjustbox}[2011/08/13]
\usepackage[bottom]{footmisc}
% \usepackage{fixltx2e}

\def\invcircledast#1{%
  \mathbin{\vphantom{\circledast}\text{%
    \ooalign{\smash{\blackcircle}\cr
             \hidewidth\smash{\textcolor{white}{\bf \footnotesize $#1$}}\hidewidth\cr
            }%
  }}%
}

\newcommand{\blackcircle}{\raisebox{-.6ex}{\scalebox{2.30}{$\bullet$}}}

% \newcommand{\Design}{$\mathsf{IM}\mathsf{HD}\xspace$}


\usepackage{etoolbox}
% \apptocmd{\thebibliography}{\scriptsize}{}{}
% \renewcommand{\bibfont}{\footnotesize}
\usepackage{bm}
\pagenumbering{gobble}

\let\oldbibliography\thebibliography
\renewcommand{\thebibliography}[1]{\oldbibliography{#1}
\setlength{\itemsep}{-2.5pt}} %Reducing spacing in the bibliography.
